Long Lived Particle Decays in MATHUSLA

We carefully study the decay and reconstruction of long-lived particle (LLP) decays in the proposed MATHUSLA LLP detector for the HL-LHC. Our investigations are focused on three LLP benchmark models. MATHUSLA's primary physics target is represented by hadronically decaying LLPs with mass above $\sim$ $10~\mathrm{GeV}$, produced in exotic Higgs decays. We also investigate GeV-scale scalar and right-handed-neutrino LLPs, which are the target of many other proposed experiments. We first introduce a public MATHUSLA FastSim code to allow for efficient signal-only studies of LLP decays in MATHUSLA and general external LLP detectors. For each of our benchmark scenarios, we carefully simulate LLP production and decay, and make our simulation library publicly accessible for future investigations and comparisons with other experiments. We then systematically study the geometric acceptance of MATHUSLA for LLP decays in these scenarios, and present updated sensitivity projections that include these acceptances. Our results show that the idealized reach of MATHUSLA computed in earlier studies is mostly realized. We also investigate possible ways of increasing the signal acceptance using the inherent geometric flexibility of the FastSim, which will provide useful inputs for realistic experimental and engineering optimization of the detector in the future.

==> changes.tex <==
v1 to v2:

added fcc LLP detector refs in intro
added compute canada acknowledgement

in response to PRD referee report:
a  bunch of tweaks and clarifications, no changes to analysis or conclusions.

